Rethinking Experience Replay: a Bag of Tricks for Continual Learning

In Continual Learning, a Neural Network is trained on a stream of data whose distribution shifts over time. Under these assumptions, it is especially challenging to improve on classes appearing later in the stream while remaining accurate on previous ones. This is due to the infamous problem of catastrophic forgetting, which causes a quick performance degradation when the classifier focuses on learning new categories. Recent literature proposed various approaches to tackle this issue, often resorting to very sophisticated techniques. In this work, we show that naive rehearsal can be patched to achieve similar performance. We point out some shortcomings that restrain Experience Replay (ER) and propose five tricks to mitigate them. Experiments show that ER, thus enhanced, displays an accuracy gain of 51.2 and 26.9 percentage points on the CIFAR-10 and CIFAR-100 datasets respectively (memory buffer size 1000). As a result, it surpasses current state-of-the-art rehearsal-based methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> authresp.tex <==
\newpage
\onecolumn
\section*{Authors' Response}
We would like to thank the reviewers and the associate editor for their useful suggestions.

\subsection*{Experiments on CORe50}
As per R1's recommendations, we integrated the experiments in Sec.~\ref{sec:exp} with tests on the more realistic CORe50 dataset. We found that the results of this experiment are in line with the ones on CIFAR-10/100: equipping Experience Replay with our tricks leads to remarkable and SOTA performances.

\subsection*{On the motivation of this paper and the rationale of the experiments}
As correctly stated by R4, the primary purpose of this paper is to serve as a quick reference for Continual Learning practitioners, providing a collection of methods for substantially improving rehearsal and non-rehearsal methods. While R1, R3 and R4 indicate that this might have limited novelty in terms of theoretical contributions, the prominent results of Sec.~\ref{subsec:stoa} show that the combination of the presented \textit{tricks} effectively allows a simple baseline to overcome state-of-the-art methods. We highlight the importance of such an experimental finding, which could motivate future works to design new accurate CL methods. Accordingly, we revised the final part of Sec.~\ref{sec:intro} and included a list of our contributions. 

\subsection*{Improved References and Explanations for the tricks}
In accordance with the suggestions of R1 and R3, we introduce further references that can clarify how tricks relate to existing literature. Briefly, as already stated, \textit{BiC} was previously published in~\cite{wu2019large}; however, differently from it, we do not need a dedicated validation set for training \textit{BiC}, but instead leverage the already-existing rehearsal memory buffer. On the other hand, \textit{IBA} \textit{(formerly DAB)}, \textit{ElrD}, \textit{BRS} and \textit{LARS} are novel. Although \textit{BRS} and \textit{LARS} are possibly similar in spirit to~\cite{aljundi2019gradient}, the latter is affected by a much higher computational overhead. With reference to these two tricks, we further clarified the explanation by adding references to the line numbers of Alg.~\ref{alg:balancoir} and~\ref{alg:lossoir} and by adding Fig.~\ref{fig:coresets} as suggested by R3.

Moreover -- after our first submission -- new research was made public by \textit{DeepMind}~\cite{mirzadeh2020understanding}, further justifying the effectiveness of learning rate decay in Continual Learning. The authors claim that this is a valuable technique allowing the network to attain flat task minima (promoted by large initial learning rates) while preventing excessive model weight displacement between tasks (due to the decay). We believe that this work provides further credibility to our proposed approaches.

\subsection*{On the use of Data Augmentation and the Independent Buffer Augmentation trick}
We put additional effort into clarifying the use of Data Augmentation in our paper, since we believe it was possibly misunderstood by R1. As the reviewer correctly points out, Data Augmentation is an obvious training expedient: indeed, we always augment the input data-stream for our experiments when using CNNs.

However, the point of the \textit{Data Augmentation on Buffer Datapoints} trick in Sec.~\ref{subsec:mem_aug} (here renamed to \textit{Independent Buffer Augmentation (IBA)} for clarity), is to independently re-augment exemplars that are drawn for replay, thus rehearsing on slightly different versions of the same input element. We respectfully disagree with R1 and believe that \textit{IBA} deserves a place in our \textit{bag of tricks}: it has a dramatic effect on accuracy and -- as reported in our reviewed Sec.~\ref{subsec:mem_aug} -- it is often neglected in widespread implementations of well-known Continual Learning methods. To provide a better understanding, we also introduced Fig.~\ref{fig:iba} showcasing the difference between augmenting on the stream and \textit{IBA}.

As requested by R1 and to further account for its importance, we also included a new experiment (Sec.~\ref{subsec:daug}) in which we apply this trick to competitors as well.

\subsection*{Additions to related works}
We thank R2 for pointing out~\cite{hou2019learning}. We added a reference to this work in Sec.~\ref{sec:related} and also contrasted its solution to the bias problem to BiC~\cite{wu2019large} in Sec.~\ref{subsec:bic}. With respect to the other references suggested by R2, we believe that they are not strictly relevant to this study, as they refer to Incremental Few-Shot Learning, which -- although related -- does not correspond to the Continual Learning setting we work on.

\subsection*{Code now available}
As R4 suggested we share further implementation details, we decided to make our code publicly available at \href{https://github.com/hastings24/mammoth_icpr/}{https://github.com/hastings24/mammoth\_icpr/}.
